WYS*: A DSL for Verified Secure Multi-party Computations

Secure multi-party computation (MPC) enables a set of mutually distrusting parties to cooperatively compute, using a cryptographic protocol, a function over their private data. This paper presents Wys*, a new domain-specific language (DSL) for writing mixed-mode MPCs. Wys* is an embedded DSL hosted in F*, a verification-oriented, effectful programming language. Wys* source programs are essentially F* programs written in a custom MPC effect, meaning that the programmers can use F*'s logic to verify the correctness and security properties of their programs. To reason about the distributed runtime semantics of these programs, we formalize a deep embedding of Wys*, also in F*. We mechanize the necessary metatheory to prove that the properties verified for the Wys* source programs carry over to the distributed, multi-party semantics. Finally, we use F*'s extraction to extract an interpreter that we have proved matches this semantics, yielding a partially verified implementation. Wys* is the first DSL to enable formal verification of MPC programs. We have implemented several MPC protocols in Wys*, including private set intersection, joint median, and an MPC card dealing application, and have verified their correctness and security.

==> lstfstar.tex <==

\lstdefinelanguage{fstar}{%
  basicstyle=\footnotesize,
  morekeywords=[1]{type,and,val,fun,let,in,ref,try,if,then,else,match,with,open,module,rec,end,assume,private,when,forall,ghost,assert,logic,array,pattern,effect,requires,ensures,decreases,modifies,fix,effect,kind},
  morekeywords=[2]{WP, Post, Pre, PURE, DIV, STATE, EXN, ALL, TotST, M, GHOST, BAD, GTot, Wys, ST, Ghost, Tot},
  morekeywords=[3]{},
  morekeywords=[4]{},
  morekeywords=[5]{Map, as_par, as_sec, as_gmw, as_rpc, mkmap_s, project, unbox_p, unbox_s, mkwire_p, mkwire_s, projwire_p, projwire_s, concat_wire, reveal, hide, unseal, sealed, seal, ffi, mkmap_p, mkmap_s, concat, Map, Sh, comb_sh, mk_sh, v_of_sh, ps_of_sh, can_sh, mkmap},
  morestring=[b]",
  sensitive=true,%
  numbersep=4pt,
%  numbers=left,
  columns=[l]fullflexible,
  texcl=true,
  mathescape=true,
%  xleftmargin=10pt,
  identifierstyle={\sffamily},
  keywordstyle=[1]{\sffamily\maybecolor{dkblue}},
  keywordstyle=[5]{\sffamily\maybecolor{dkred}},
  keywordstyle=[2]{\sffamily\maybecolor{dkblue}},
  keywordstyle=[3]{\maybecolor{dkred}},
  keywordstyle=[4]{\rmfamily\itshape},
% Here is the range marker stuff
  rangeprefix=(*---\ ,
  includerangemarker=false,
  stringstyle=\ttfamily,
  showspaces=false,
  moredelim=[is][\sffamily\scriptsize\maybecolor{blue}]{~}{~},
  morecomment=[n]{(*}{*)},
  commentstyle={\itshape\maybecolor{dkred}},
  literate={->}{$\rightarrow\,$}{1}
	   {delta}{$\delta$}{1}
	   {exists}{$\exists$}{1}
	   {forall}{$\forall$}{1}
	   {/\\}{$\wedge\;$}{1}
	   {\\/}{$\vee\;$}{1}
           {>=}{$\geq\ $}{2}
           {<=}{$\leq\ $}{2}
	   {<==>}{$\Longleftrightarrow \ $}{3}
	   {==>}{$\Longrightarrow \ $}{3}
     {--}{-}{1}   % Added due to         - not displaying properly.  Weird. ... but may make arrows look bad  {...}{$\ldots$}{3}
     {<<}{$\prec\ $}{1}
           ,
  breaklines=false}

